Predicting Topological Maps for Visual Navigation in Unexplored Environments

We propose a robotic learning system for autonomous exploration and navigation in unexplored environments. We are motivated by the idea that even an unseen environment may be familiar from previous experiences in similar environments. The core of our method, therefore, is a process for building, predicting, and using probabilistic layout graphs for assisting goal-based visual navigation. We describe a navigation system that uses the layout predictions to satisfy high-level goals (e.g. "go to the kitchen") more rapidly and accurately than the prior art. Our proposed navigation framework comprises three stages: (1) Perception and Mapping: building a multi-level 3D scene graph; (2) Prediction: predicting probabilistic 3D scene graph for the unexplored environment; (3) Navigation: assisting navigation with the graphs. We test our framework in Matterport3D and show more success and efficient navigation in unseen environments.

==> latex/content/conclusion.tex <==

\section{Conclusion}
\label{sec:conclusion}

Abstract-level goal-directed navigation and exploration is an important task in robot navigation, especially in unexplored but familiar environments.
% To the best of our knowledge, we are the first to propose a framework and a simulator for high-level goal-directed visual navigation in a topological map.
We adopt a topological representation (layout graph) to encode the environment structure.
The topological graph is served as the centerpiece of our three-stage framework, including Perception and Mapping, Prediction, and Navigation.
We propose a navigation framework with a mixture of learning-based models and rule-based mechanisms.
The proposed approach is extensively studied and tested using the Matterport3D dataset.
We specifically test our framework on REVERIE task, which is similar to our application scenarios.
Our results show that learning the proposed framework is helpful in assisting robot navigation in unexplored environments.

==> latex/fig_tab_alg/fig_graph_pred_eg.tex <==
\begin{figure}[t!]
        \centering
		\includegraphics[width=0.9\columnwidth]{latex/fig_tab_alg/figures/graph_pred_eg.pdf}
		\vspace{-10pt}
		\caption{
		    Graph prediction example. We pre-define a route (From ``dining" to ``toilet") and the graph prediction result at each step is shown.
		    \textbf{Node: } Description in green means predicted nodes. Only the class with highest probability is shown above for visualization purpose.
		    \textbf{Edge:} Dash lines means predicted edges.
		}
		\label{fig:graph_pred_eg}
		\vspace{-20pt}
\end{figure}


==> latex/fig_tab_alg/fig_mp3d.tex <==
\begin{figure*}[t!]
        \centering
		\includegraphics[width=1\textwidth]{latex/fig_tab_alg/figures/mp3d_eg.pdf}
% 		\vspace{-20pt}
		\caption{
		    Matterport3D dataset examples. 
		    \textbf{(1)}:
		    Panorama connectivity graph
		  %  \citep{mattersim}
		    \textbf{(2)}:
		    Intra/Inter-region panorama connectivity graph. Yellow edges represent the connectivity between panoramas at different regions.
		    \textbf{(3)}:
		    Region connectivity graph built from (2). Each node represents a region, and the yellow edges represent the traversibility between regions. 
		}
		\label{fig:mp3d}
		\vspace{-15pt}
\end{figure*}

==> latex/fig_tab_alg/fig_teaser.tex <==
\begin{figure}[t!]
        \centering
		\includegraphics[width=1\columnwidth]{latex/fig_tab_alg/figures/teaser.pdf}
		\vspace{-3em}
		\caption{Our agent maintains a scene graph and predict the unexplored environment condition on the observation graph and a destination instruction (``Go to Kitchen"). The ``imagined" scene graph is used as a prior to help the agent in navigation decision making process.
		In this example, orange/white/green nodes represent visited/current/predicted regions respectively.
		}
		\label{fig:teaser}
		\vspace{-8pt}
\end{figure}

==> latex/fig_tab_alg/tab_ablation2.tex <==
% 
\begin{table*} [t]  
    \begin{center}
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{ | l |  c  c | c c | } 
        \hline
        \multirow{2}*{\textbf{Experiments}} &
        \multicolumn{2}{c|}{\textbf{Val Unseen}} 
        % \multicolumn{2}{c|}{\textbf{GT in}} 
        \\
        % & SR & SPL
        & SR & SPL \\
        \hline
        \hline
        Baseline 
        % & 49.5 & 45.1 
        & 27.4 & 23.1 \\
        
        Baseline, 50epi
        % & 50.3 & 45.3 
        & 27.9 & 23.2 \\
        
        [$\textbf{G}$]-informed
        % & 51.0 & 46.0 
        & 29.8 & 24.2 \\
        
        [$\textbf{G}$, $\textbf{P}$]-informed 
        % & 51.0 & 46.0 
        & 30.6 & 24.4  \\
        
        [$\textbf{G}$, $\textbf{M}$]-informed
        % & 50.8 & 45.9 
        & 29.7 & 25.3 \\
        
        [$\textbf{G}$, $\textbf{P}$, $\textbf{M}$]-informed
        % & 50.0 & 45.7 
        & 31.8 & 26.1  \\
        
        [$\textbf{G}$, $\textbf{P}$, $\textbf{M}$]-informed, 50epi
        % & 51.5 & 46.1 
        & 33.3 & 26.5 \\
        
        \hline
        \hline
        \multicolumn{3}{|c|}{Ground-Truth information involved} \\
        \hline
        
        
        [$\textbf{G}^*$]-informed
        % & 51.5 & 46.6 
        & 31.0 & 25.5 \\
        
        [$\textbf{G}$, $\textbf{P}^*$]-informed 
        % & 51.0 & 46.0 
        & 33.1 & 26.1 \\
        
        % [$\textbf{G}^*$, $\textbf{P}^*$]-informed 
        % % & 54.3 & 48.2 
        % & 34.3 & 27.6 \\
        
        [$\textbf{G}$, $\textbf{P}^*$]-informed, 50epi
        & 34.5 & 26.3 \\
        
        % [$\textbf{G}^*$, $\textbf{P}^*$]-informed 
        % & 54.3 & 48.2 & 34.3 & 27.6 \\
        
        [$\textbf{G}$, $\textbf{P}^*$, $\textbf{M}$]-informed 
        % & 56.0 & 49.5 
        & 37.9 & 29.4 \\
        
        [$\textbf{G}$, $\textbf{P}^*$, $\textbf{M}$]-informed, 50epi
        % & 60.6 & 50.6 
        & 45.1 & 30.1 \\
        
        % [$\textbf{G}^*$, $\textbf{P}^*$, $\textbf{M}$]-informed, 50epi
        % % & 63.2 & 50.5 
        % & 47.5 & 31.2 \\
        
        
        % % partial gt
        % [$\textbf{G}^*$, $\textbf{P}^#$, $\textbf{M}$]-informed, 50epi
        % &  &  &  &  \\
        
        \hline
    \end{tabular}
    }
    \end{center}
    \vspace{-1em}
    \caption{
        Ablation studies. 
        $\textbf{G}^*$/$\textbf{G}$: GT/predicted subgoal token is used; 
        $\textbf{P}^*$/$\textbf{P}$: GT Perception/Perception model is used; 
        $\textbf{M}$: Map-informed exploration is used; 
        50epi: maximum 50 episodes.
    }
    \label{table:exp:ablation}
\end{table*}
% % 


==> latex/fig_tab_alg/tab_localization.tex <==
%
% \begin{table} %{r}{0.3\columnwidth}  
    \begin{center}
    \resizebox{0.3\columnwidth}{!}
    {%
    \begin{tabular}{ l |  c  }
        \hline
        Variants &
        Accuracy
        \\
        \hline
        no pose & 76.37
        \\
        no encoding & 77.38
        \\
        w/ encoding (L=5) & 78.15
        \\
        \hline
        \end{tabular}
    }
    \end{center}
    \caption{Ablation study for the Localization model regarding camera pose encoding}
    \label{table:exp:localization}
    % \vspace{10pt}
% \end{table}
% 
